Causality and Responsibility for Formal Verification and Beyond

The theory of actual causality, defined by Halpern and Pearl, and its quantitative measure - the degree of responsibility - was shown to be extremely useful in various areas of computer science due to a good match between the results it produces and our intuition. In this paper, I describe the applications of causality to formal verification, namely, explanation of counterexamples, refinement of coverage metrics, and symbolic trajectory evaluation. I also briefly discuss recent applications of causality to legal reasoning.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{G. G\"ossler and O. Sokolsky (Eds.): 1st Workshop on Causal Reasoning for \\ Embedded and safety-critical Systems Technologies (CREST'16)\\
EPTCS 224, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.224.1}{10.4204/EPTCS.224.1}}
\pdfoutput=1

